Measuring Fairness of Text Classifiers via Prediction Sensitivity

With the rapid growth in language processing applications, fairness has emerged as an important consideration in data-driven solutions. Although various fairness definitions have been explored in the recent literature, there is lack of consensus on which metrics most accurately reflect the fairness of a system. In this work, we propose a new formulation : ACCUMULATED PREDICTION SENSITIVITY, which measures fairness in machine learning models based on the model's prediction sensitivity to perturbations in input features. The metric attempts to quantify the extent to which a single prediction depends on a protected attribute, where the protected attribute encodes the membership status of an individual in a protected group. We show that the metric can be theoretically linked with a specific notion of group fairness (statistical parity) and individual fairness. It also correlates well with humans' perception of fairness. We conduct experiments on two text classification datasets : JIGSAW TOXICITY, and BIAS IN BIOS, and evaluate the correlations between metrics and manual annotations on whether the model produced a fair outcome. We observe that the proposed fairness metric based on prediction sensitivity is statistically significantly more correlated with human annotation than the existing counterfactual fairness metric.

==> Sensitivity_ACL (7)/archive.tex <==

\section{Determining Protected Attribute Tokens}
\label{section:psm}

A major challenge remains in applying prediction sensitivity to measure individual fairness: it is unclear what the optimal method is in determining protected attribute tokens. Bias in language models arises from subtle correlations between our societal biases and the language features that result from them.

We propose an extension---called \emph{weighted prediction sensitivity}---to address this challenge and capture these correlations. Our approach involves training an \emph{additional} model to \emph{predict} the protected status of an individual, and then weighting the feature attribution scores of the target model's prediction according to these results.


==> Sensitivity_ACL (7)/results_bib.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{p{7cm}p{1cm}p{1cm}|p{1cm}p{1cm}p{1cm}p{1cm}p{0.9cm}}
%\toprule
%\multirow{1}{*}{Individual Fairness Metrics} & \multicolumn{3}{l}{Point-biserial correlation ($\downarrow$)} & \multicolumn{4}{l}{ Mutual Information ($\downarrow$)} \\
%\midrule
% & BiB & JT(G) & JT(R) & BiB & JT(G) & JT(R) & JT(GR)  \\ \cline{2-8}
%P1 (uniform $\bm w, \bm v$) & 0.206 & 0.117 & 0.064 & 0.013 & 0.007 & 0.009 & 0.011 \\ 
%CF \cite{garg2019counterfactual} & 0.326 & 0.214 & 0.098 & 0.025 & 0.022 & 0.015 & 0.029  \\ 
%P4 ($\bm v$ set using gendered words) & 0.34 & 0.227 & 0.102 & 0.037 & 0.054 & 0.007 & 0.031 \\ 
%P5 ($\bm v$ set using gendered words and embedding vectors) & \textbf{0.363} & 0.295 & 0.108 & \textbf{0.098} & 0.061 & 0.027 & 0.042 \\ 
%P2 ($\bm v$ set using PSM)& \textbf{0.397} & 0.358 & 0.113 & \textbf{0.102} & \textbf{0.097} & 0.021 & 0.077 \\ 
%P3  ($\bm v$ set using PSM and embedding vectors) & \textbf{0.441} & \textbf{0.374}& 0.101 & \textbf{0.105} & \textbf{0.101} & 0.038 &0.084\\ 
%\bottomrule

\toprule
\multirow{1}{*}{Individual Fairness Metrics} & \multicolumn{2}{c|}{Bias in Bios} & \multicolumn{2}{c}{Jigsaw Toxicity} \\
\midrule
 & Corr. & MI & Corr. & MI  \\ \cline{2-5}
P1 (uniform $\bm w, \bm v$) & 0.206 & 0.013 & 0.117 & 0.007 \\ 
CF \cite{garg2019counterfactual} & 0.326 & 0.025 & 0.214 & 0.022  \\ 
P4 ($\bm v$ set using gendered words) & 0.34 & 0.037 & 0.227 & 0.054 \\ 
P5 ($\bm v$ set using gendered words and embedding vectors) & \textbf{0.363} & \textbf{0.098} & 0.295 & 0.061  \\ 
P2 ($\bm v$ set using PSM)& \textbf{0.397} & \textbf{0.102} & 0.358 &  \textbf{0.097}  \\ 
P3  ($\bm v$ set using PSM and embedding vectors) & \textbf{0.441} & \textbf{0.105}&  \textbf{0.374} &  \textbf{0.101} \\ 

%Numbers with Bios in Bias PSM (Male test set accuracy : 98.84, Female test set accuracy : 98.17)
%Numbers with Jigsaw Toxicity PSM (Male test set accuracy : 95.52, Female test set accuracy : 96.22)



\bottomrule

\end{tabular}
\caption{\label{citation-guide} Point bi-serial correlations (Corr.) and Mutual Information (MI) between different individual fairness metrics with human annotations on Bios in Bias and Jigsaw toxicity datasets. Bold numbers are the correlations where we see statistically significant increase over CF baseline. The metric variants are sorted based on the correlation values. We use the bootstrap method to compute statistical significance \cite{koehn2004statistical} at p-value<0.05.}
\label{tab:table1}
\end{table*}




==> Sensitivity_ACL (7)/results_jigsaw.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{p{6cm}p{2cm}p{3cm}}
%\hline \textbf{Model} &   \textbf{Raw task AUC} & \textbf{TPED} & \textbf{CRA} \\
\toprule
\multirow{1}{*}{Individual Fairness Metrics} & {Point-biserial correlation ($\downarrow$)} & { Mutual Information ($\downarrow$)} \\
\midrule
P1 (uniform $\bm w, \bm v$) & 0.117 &  0.007   \\
CF \cite{garg2019counterfactual} &   0.214  & 0.022 \\
P4 ($\bm v$ set using gendered words) &  0.227 &  0.054  \\
P5 ($\bm v$ set using gendered words and embedding vectors) &  0.295 &  0.061  \\
P2 ($\bm v$ set using PSM) &  0.358 &  \textbf{0.097}  \\
P3  ($\bm v$ set using PSM and embedding vectors) &  \textbf{0.374} &  \textbf{0.101}  \\
\bottomrule
\end{tabular}
\caption{\label{font-table} Table showing correlations between different individual fairness metrics with human annotations on Jigsaw Toxicity dataset.  Bold numbers are the correlations where we see statistically significant increase over CF baseline}
\label{table:table2}
\end{table*}

==> archive.tex <==

\section{Determining Protected Attribute Tokens}
\label{section:psm}

A major challenge remains in applying prediction sensitivity to measure individual fairness: it is unclear what the optimal method is in determining protected attribute tokens. Bias in language models arises from subtle correlations between our societal biases and the language features that result from them.

We propose an extension---called \emph{weighted prediction sensitivity}---to address this challenge and capture these correlations. Our approach involves training an \emph{additional} model to \emph{predict} the protected status of an individual, and then weighting the feature attribution scores of the target model's prediction according to these results.


==> results_jigsaw.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{p{6cm}p{2cm}p{3cm}}
%\hline \textbf{Model} &   \textbf{Raw task AUC} & \textbf{TPED} & \textbf{CRA} \\
\toprule
\multirow{1}{*}{Individual Fairness Metrics} & {Point-biserial correlation ($\downarrow$)} & { Mutual Information ($\downarrow$)} \\
\midrule
P1 (uniform $\bm w, \bm v$) & 0.117 &  0.007   \\
CF \cite{garg2019counterfactual} &   0.214  & 0.022 \\
P4 ($\bm v$ set using gendered words) &  0.227 &  0.054  \\
P5 ($\bm v$ set using gendered words and embedding vectors) &  0.295 &  0.061  \\
P2 ($\bm v$ set using PSM) &  0.358 &  \textbf{0.097}  \\
P3  ($\bm v$ set using PSM and embedding vectors) &  \textbf{0.374} &  \textbf{0.101}  \\
\bottomrule
\end{tabular}
\caption{\label{font-table} Table showing correlations between different individual fairness metrics with human annotations on Jigsaw Toxicity dataset.  Bold numbers are the correlations where we see statistically significant increase over CF baseline}
\label{table:table2}
\end{table*}
